GSDF: 3DGS Meets SDF for Improved Rendering and Reconstruction

Presenting a 3D scene from multiview images remains a core and long-standing challenge in computer vision and computer graphics. Two main requirements lie in rendering and reconstruction. Notably, SOTA rendering quality is usually achieved with neural volumetric rendering techniques, which rely on aggregated point/primitive-wise color and neglect the underlying scene geometry. Learning of neural implicit surfaces is sparked from the success of neural rendering. Current works either constrain the distribution of density fields or the shape of primitives, resulting in degraded rendering quality and flaws on the learned scene surfaces. The efficacy of such methods is limited by the inherent constraints of the chosen neural representation, which struggles to capture fine surface details, especially for larger, more intricate scenes. To address these issues, we introduce GSDF, a novel dual-branch architecture that combines the benefits of a flexible and efficient 3D Gaussian Splatting (3DGS) representation with neural Signed Distance Fields (SDF). The core idea is to leverage and enhance the strengths of each branch while alleviating their limitation through mutual guidance and joint supervision. We show on diverse scenes that our design unlocks the potential for more accurate and detailed surface reconstructions, and at the meantime benefits 3DGS rendering with structures that are more aligned with the underlying geometry.

==> secs/preliminary.tex <==
\section{Preliminary}
In this section, we will briefly discuss two techniques employed in our method, which sets the foundation for our two-branch structures.

\subsection{Neural volume rendering of SDF}
Neural volume rendering \cite{mildenhall2020nerf} implicitly represents 3D scenes as continuous fields from calibrated multi-view images. However, the density-based representation can not accurately present the scene geometry. The signed distance function (SDF) also represents a continuous field and is widely used to reconstruct accurate geometry from 3D point cloud~\cite{Boulch_2022_CVPR, kazhdan2006poisson, zhao2021progressive, Park_2019_CVPR}. The potential surface can be extracted in the zero-level set of SDF field using Marching Cube~\cite{lorensen1998marching}.  To reconstruct accurate geometry models from multi-view images, Neus \cite{wang2021neus} introduced the signed distance function (SDF) to the Neural Radiance Fields by converting the volume density to SDF with a logistic function:
\begin{equation}
\alpha_i=\max \left(\frac{\Phi_s\left(f\left(\mathbf{x}_i\right)\right)-\Phi_s\left(f\left(\mathbf{x}_{i+1}\right)\right)}{\Phi_s\left(f\left(\mathbf{x}_i\right)\right)}, 0\right),
\end{equation}
where $\Phi_s$ denotes a Sigmoid function and $f(x)$ denotes the SDF value of position $x$. Following the classical volume rendering scheme, the predicted color of a ray $r$ by accumulating alphas and colors of the sample points:
\begin{equation}
\hat{\mathbf{C}}(\mathbf{r})=\sum_{i=1}^P T_i \alpha_i \mathbf{c}_i, T_i=\exp \left(-\sum_{j=1}^{i-1} \alpha_j \delta_j\right),
\end{equation}
where $\delta_j$ is the distance between adjacent sampled points. In our method, we build the reconstruction branch based on Instant-nsr~\cite{instant-nsr-pl}, which uses a multi-level hash grid~\cite{muller2022instant} to store the features of the scenes. Furthermore, the multi-level hash grid is progressively trained from low-level to high-level as~\cite{li2023neuralangelo} to make the SDF field optimized from coarse to fine and avoid falling into local minima. 




% Compared to density-based volume rendering, SDF-based volume rendering provides a clearer definition of surface extraction, \ie, the zero-level set of the SDF $\mathcal{S}=\left\{\mathbf{x} \in \mathbb{R}^3 \mid f(\mathbf{x})=0\right\}$, allowing for more precise geometry extraction. Neus \cite{wang2021neus} represents a 3D scene as a signed distance field $f(x): \mathbb{R}^3 \rightarrow \mathbb{R_{+}}$ and a radiance field $c(x,d): \mathbb{R}^3 \times \mathbb{S}^2 \rightarrow \mathbb{R}^3$, where $x$ denotes a spatial position and $d$ denotes the view direction respectively. 
% To convert SDF value into opacity $\alpha_i$ of each point $x_i$ for volume rendering, Neus leverages the logistic function: 

% \begin{equation}
% \alpha_i=\max \left(\frac{\Phi_s\left(f\left(\mathbf{x}_i\right)\right)-\Phi_s\left(f\left(\mathbf{x}_{i+1}\right)\right)}{\Phi_s\left(f\left(\mathbf{x}_i\right)\right)}, 0\right),
% \end{equation}

% where $\Phi_s$ denotes a sigmoid function. Following the classical volume rendering scheme, we compute the color of a ray $r$ by accumulating alphas and colors of the sample points:
% $\hat{\mathbf{C}}(\mathbf{r})=\sum_{i=1}^P T_i \alpha_i \mathbf{c}_i,$ where $T_i=\exp \left(-\sum_{j=1}^{i-1} \alpha_j \delta_j\right)$ and $\delta_j$ is the distance between adjacent sampled points.

\subsection{3D gaussian splatting and variants}

\paragraph{3D Gaussian Splatting (3D-GS).} 3D-GS \cite{kerbl20233d} explicitly represents the whole 3D scene using 3D Gaussians, where each Gaussian is defined by the mean $\mu \in \mathbb{R}^3$ and the covariance $\Sigma \in \mathbb{R}^{3 \times 3}$:

\begin{equation}
    G(x)=e^{-\frac{1}{2}(x-\mu)^T \Sigma^{-1}(x-\mu)},
\end{equation}
where x is the any space location. To guarantee positive semi-definite, 3D covariance $\Sigma$ is formulated by a scaling matrix $S$ and a rotation matrix $R$.
Furthermore, an opacity value $\alpha \in \mathbb{R}$ and a color feature $c \in \mathbb{R}^C$ are also maintained for modeling view dependent effects by Spherical harmonics. For novel view synthesis, 3D-GS employs tile-based rasterization rather than traditional volume rendering. Specifically, it projects 3D Gaussians onto the image plane as 2D Gaussians, sorts them in front-to-back depth order and performs $\alpha$-blending for each pixel.

\paragraph{Scaffold-GS.} \cite{scaffoldgs}.



